SoK: Vehicle Orientation Representations for Deep Rotation Estimation

In recent years, there is an influx of deep learning models for 3D vehicle object detection. However, little attention was paid to orientation prediction. Existing research work proposed various vehicle orientation representation methods for deep learning, however a holistic, systematic review has not been conducted. Through our experiments, we categorize and compare the accuracy performance of various existing orientation representations using the KITTI 3D object detection dataset, and propose a new form of orientation representation: Tricosine. Among these, the 2D Cartesian-based representation, or Single Bin, achieves the highest accuracy, with additional channeled inputs (positional encoding and depth map) not boosting prediction performance. Our code is published on GitHub: https://github.com/umd-fire-coml/KITTI-orientation-learning

==> todo.tex <==

- new section for loss functions in general
- Table to compare loss functions

- Adding more papers to each of the representations (likely single bin/single value) (20-30 reference)

1. Introduction:
What is monocular object detection?
 - weaknesses compared to LiDAR and stereo based vehicle objection
      - LiDAR is sparse and requires heavy computation to learn 3D represetations for objects
      - Stereo estimation can derive depth, motion?, ... to make orientation estimation much easier
      
 - vehicle only -> other classes require many more features to learn representation, so to compare orientation representations only, we restrict our domain of interest to vehicles.
 
 What's Kitti dataset?
  - limitation for rotation Degree of Freedom
  - Edge cases: car climbing a ramp
  
 What are challenges for orientation estimation?
 - discontinuity 
 - ambiguity
 


Monocular only:
pros:
 - all our experiments are monocular based
 - motivation for our problem is clearer
cons:
 - how do we explain consideration of non-monocular tasks?
    - LiDAR is still hard
    - stereo is much easier <- "Survey of Vehicle Orientation Representations for Monocular Deep Rotation Estimation"
    
2. Related work: 
 moving current section to Vehicle orientation representation
 % \section{Related Works}
% %Create a table of papers and the orientation learning technique.


% % cite a bunch of 3D Object Detection or 3D Rotation Estimation papers that performs orientation learning, group them together if they are done similarity, separate them out if it is unique. 

% % cite papers that used scalar method
% Although Grassia~\cite{grassia1998practical} states that Euler angles and quaternions representation are not ideal to compute and differentiate positions, because of the representation can have \textit{discontinuity} at $\pm180^{\circ}$ and the representation is \textit{ambiguous} as there are multiple “correct” orientations for each object\cite{saxena2009learning}, we still observe recent researchers such as \cite{chen2021monorun, wang2021depth, park2021pseudo} using these types of scalar-based angle representation in 3D Object Detection. To alle Wang et al. \cite{wang2021fcos3d} claimed better performance when dividing the angles into 2-bins with each bin represented by angle $\theta$ (offset) with period $\pi$. However, such methods can still suffer from \textit{discontinuity} and \textit{ambiguity} problem for values at the border of each bin.

% %cite papers that use the axis, heading, offset 3 value method.
% Kumar et al.  \cite{kumar2021groomed} 

%cite papers that use the (cos, sin), or cos method
% The discontinuity problem can be partly resolved by representing the angle using the cosine of the angle \cite{he2020svga, zheng2021se, reading2021categorical, lang2019pointpillars} due to its periodic properties. However, cosine of the angle cannot be unambiguously converted back into the angle without using at least 3-bins. Furthermore, when the angular difference $\delta = \pm\pi$, the differentiation results of $cos(\delta)$ are zero, which could stop backpropagation learning at the extreme opposite output. To resolve this problem, researchers \cite{Liu_2020_CVPR_Workshops,deng2020voxel,liu2021ground,shi2021geometry} performed regression on both the cosine and sine of the angle (cos($\theta$), sin($\theta$)). 

% cite papers that use the multi-bin, or multi affinity method
% Liao et al. \cite{liao2019spherical} stated that converting challenges with continuous nature to classification problem lead to stable training and convergence. They proposed that gradient updates are not constrained in regression while the classification task has restricted gradient updates due to the nature of the softmax layer in the end. As Inspired by MultiBin \cite{multibin_mousavian_2017}, multiple papers \cite{chen2020monopair, zhou2019objects, zhang2021learning, ma2021delving, Chen_2016_CVPR, ku2019monocular,gs3d_li_2019,liu2019deep} divide orientation into different bins and predict them as categorical problem. The idea of discrete bins has a trade-off between the number of bins and coverage of the bins, so final angle prediction accuracy depends on the number of bins and specific implementations.
 
 % \subsection{4-Bins with Confidence (Confidence Bins) vs 4-Bins without Confidence (Voting Bins)}
% \begin{figure}[h!]
%         \centering
%         \includegraphics[width=100mm]{diagrams/experiment_result/bin_with_confi.pdf}
%         \caption{Validation Accuracy of bins with confidence (4-bin multibins) and bins without confidence (4-bin voting bin)}
%         \label{fig:bins_with_conf}
%     \end{figure}
%     \begin{table}[h!]
%         \centering
%         \begin{tabularx}{\textwidth} { 
%             | 
%             >{\centering\arraybackslash}X | 
%             >{\centering\arraybackslash}X | 
%             >{\centering\arraybackslash}X | }
%             \hline
%             Method   &  Num of Bins    & Accuracy (\%) \\ 
%             \hline\hline
%             Confidence Bins   & 4-bins        & 88.071 \\
%             Voting Bins  & 4-bins        & 93.609 \\
%             \hline
%         \end{tabularx}
%         \caption{Highest validation accuracy of 4-bin Multibin and Voting Bins}
%         \label{table:bins_with_conf}
%     \end{table}
 Introduction:
 - Look at the bullet points in the introduction

N-Dim: move mean-shift affinity
Metrics: redo, we don't use AOS similarity, as we are not predicting bounding boxes.


12/04:
Reorganize section 2.3
Talk about loss function: multibin uses l2 loss
Talk about section 4.5 Angular loss vs L2 loss
Talk about section 4.6  multibin vs voting bin
Multibin or Conf bins?

What's wrong with our multibin???


13 images 17 pages without reference


